Beyond The Text: Analysis of Privacy Statements through Syntactic and Semantic Role Labeling

This paper formulates a new task of extracting privacy parameters from a privacy policy, through the lens of Contextual Integrity, an established social theory framework for reasoning about privacy norms. Privacy policies, written by lawyers, are lengthy and often comprise incomplete and vague statements. In this paper, we show that traditional NLP tasks, including the recently proposed Question-Answering based solutions, are insufficient to address the privacy parameter extraction problem and provide poor precision and recall. We describe 4 different types of conventional methods that can be partially adapted to address the parameter extraction task with varying degrees of success: Hidden Markov Models, BERT fine-tuned models, Dependency Type Parsing (DP) and Semantic Role Labeling (SRL). Based on a detailed evaluation across 36 real-world privacy policies of major enterprises, we demonstrate that a solution combining syntactic DP coupled with type-specific SRL tasks provides the highest accuracy for retrieving contextual privacy parameters from privacy statements. We also observe that incorporating domain-specific knowledge is critical to achieving high precision and recall, thus inspiring new NLP research to address this important problem in the privacy domain.

==> dataset.tex <==
%!TEX root = main.tex
\section{Dataset}

We present analysis of the privacy policy annotations. 

We examine which privacy statement are more compatible with our approach.

==> discussion.tex <==
%!TEX root = main.tex
\section{Discussion}

The CI annotation of privacy policies provides a way for a statement level analysis of policies. In this paper, we describe an NLP based method to perform automatic CI annotation of privacy statements. This work has several implications for different stakeholders, some of which were discussed  in~\cite{shvartzshnaider2019going}. 

For consumers, who often find privacy policies to long and complex to read,  the CI annotation provide an ability to  queries of the privacy policies for specific flows it prescribes. These can involved asking about mentions of specific ``senders" and ``recipients" in the privacy policies, type of information being collected or shared, and listing the conditions and purposes. Beyond enumerating the prescribed CI parameters, the method enables contextual queries that reflect up to 5 CI parameters. For example, instead of asking about mentions of  ``location information," the query can include the senders, recipients of interest, such as third parties, contractors. The query can further refined to include specific constraints under which location data is transferred, e.g., when user is using the app.

The CI abstraction allows to query different privacy policies, potentially, from different sectors. It can also serve as a way to compare different versions of the same privacy policy to examine the new changes that were introduced in the new version.  We can identify which new flows were added or removed, consequently, what data types, senders, recipients, subjects and conditions were changed. 

The annotation also open an interesting avenue for visualization of the prescribed flows, in addition to the current text version. A variant of a Sankey diagram, Figure~\ref{third_party_flows}, or a more creative version, can graphically reflect the important information flows generated by different data handling practices. 

Finally, combine with existing crowdsourcing methodologies of learning users privacy expectations~\cite{apthorpe2018discovering,shvartzshnaider2016learning,apthorpe2019evaluating}, we can perform a large scale analysis of what privacy policies align with users expectations and existing societal norms.

For relevant agencies like Federal Trade Commission, the CI-based analysis of privacy policies can serve for a robust auditing technique of prescribed data handling practices. Using the CI framework, the resulting information flows can be automatically compared with existing regulation~\cite{apthorpe2019evaluating} and users privacy expectations~\cite{shvartzshnaider2016learning, apthorpe2018discovering}. Furthermore, the analysis can help detect privacy statements with missing contextual information that resulting in ambiguous flows.  Ultimately, we envision our work used as part of the overall evaluation framework for performing dynamic and static analysis of digital services, similar to ~\cite{sanfilippo2019disaster}. Specifically, the CI annotated policy fed into an automatic test suite for possible violation of privacy policy, regulation or societal expectations. 

\subsection{Limitations}

As discussed in Section~\ref{sec:Evaluation} our annotation methods results in high accuracy of annotations. Nevertheless, there are cases where our approach does not perform as well. Our evaluation with different models shows that a better SRL model coupled with domain knowledge heuristc produces improved results. Previous results~\cite{shvartzshnaider2019going} showed the crowdworkers are able to identify CI parameters with high percision.
Coupled with our approach, crowdworker can filter the false positives and increase the percision further. 






